Data-driven Signal Decomposition Approaches: A Comparative Analysis

Signal decomposition (SD) approaches aim to decompose non-stationary signals into their constituent amplitude- and frequency-modulated components. This represents an important preprocessing step in many practical signal processing pipelines, providing useful knowledge and insight into the data and relevant underlying system(s) while also facilitating tasks such as noise or artefact removal and feature extraction. The popular SD methods are mostly data-driven, striving to obtain inherent well-behaved signal components without making many prior assumptions on input data. Among those methods include empirical mode decomposition (EMD) and variants, variational mode decomposition (VMD) and variants, synchrosqueezed transform (SST) and variants and sliding singular spectrum analysis (SSA). With the increasing popularity and utility of these methods in wide-ranging application, it is imperative to gain a better understanding and insight into the operation of these algorithms, evaluate their accuracy with and without noise in input data and gauge their sensitivity against algorithmic parameter changes. In this work, we achieve those tasks through extensive experiments involving carefully designed synthetic and real-life signals. Based on our experimental observations, we comment on the pros and cons of the considered SD algorithms as well as highlighting the best practices, in terms of parameter selection, for the their successful operation. The SD algorithms for both single- and multi-channel (multivariate) data fall within the scope of our work. For multivariate signals, we evaluate the performance of the popular algorithms in terms of fulfilling the mode-alignment property, especially in the presence of noise.

==> NaveedReferences <==
%\footnotesize
\begin{thebibliography}{200} % 100 is a random guess of the total number of

\bibitem{Flandrin18} P. Flandrin, \emph{Explorations in Time-Frequency Analysis}. New York, NY: Cambridge University Press, 2018.

\bibitem{SPM20} A. M. -C. So, P. Jain, W. -K. Ma and G. Scutari, ``Nonconvex Optimization for Signal Processing and Machine Learning [From the Guest Editors],'' \emph{IEEE Signal Process. Mag.}, vol. 37, no. 5, pp. 15-17, 2020.

%
\bibitem{Cohen95} L. Cohen, \emph{Time-Frequency Analysis: Theory and Applications}. Englewood Cliffs, NJ: Prentice Hall, 1995.




%\bibitem{Fland99} P. Flandrin, \emph{Time-Frequency/Time-Scale analysis}. San Diego, CA: Academic Press, 1999.



%\bibitem{Ville48} J. Ville, ``Théorie et Applications de la Notion de Signal Analytique,'' \emph{Câbles et Transmission}, vol. 2, pp. 61–74, 1948.

\bibitem{Huang98} N. E. Huang, Z. Shen, S. R. Long, Wu, M. L., H. H. Shih, Q. Zheng, N. C. Yen, C. C. Tung, and H. H. Liu, ``The Empirical Mode Decomposition and Hilbert spectrum for nonlinear and non-stationary time series analysis,'' \emph{Proc. R. Soc. Lond. A, Math. Phys. Sci.}, vol. 454, no. 1971, pp. 903–995, 1998.

\bibitem{Daub11} I. Daubechies, J. Lu, and H. T. Wu, ``Synchrosqueezed wavelet transforms: An Empirical Mode Decomposition-like tool,'' \emph{Appl. Comput. Harmon. Anal.}, vol. 41, pp. 384-411, 2016.

\bibitem{Maragos01} A. Potamianos and P. Maragos,  ``Time-Frequency Distributions for Automatic Speech Recognition,'' \emph{IEEE Trans. Speech Audio Process.}, vol. 9, pp. 196-200, 2001.

\bibitem{Mallat08} G. Yu, S. Mallat, and E. Bacry, ``Audio denoising by time-frequency block thresholding,'' \emph{IEEE Trans. Signal Process.}, vol. 56, pp. 1830-1839. 2008.

%\bibitem{Necciari13} T. Necciari, P. Balazs, N. Holighaus, and P. Soendergaard,  ``The ERBlet transform: An auditory-based time-frequency representation with perfect reconstruction,'' \emph{Proc. IEEE Int. Conf. Acoustics, Speech, and Signal Processing (ICASSP)}, 2013.

\bibitem{Matz13} G. Matz, H. Bolcskei and F. Hlawatsch, ``Time-Frequency Foundations of Communications: Concepts and Tools,'' \emph{IEEE Signal Process. Mag.}, vol. 30, pp. 87-96, 2013.

\bibitem{Park13} C. Park, D. Looney, N. Rehman and D. P. Mandic, ``Motor imagery signal classification using multivariate empirical mode decomposition'', \emph{IEEE Trans. Neural Syst. Rehabilitation Eng.}, vol. 21, pp. 10-22, 2013.

\bibitem{Saleem19} S. Saleem, S. S. Naqvi, T. Manzoor, A. Saeed, N. Rehman, J. Mirza, ``A strategy for classification of vaginal vs. cesarean section delivery: bivariate empirical mode decomposition of cardiotocographic recordings,'' \emph{Front. Physiol.}, vol. 10, pp. 246, 2019.

\bibitem{Dybala14} J. Dybala and R. Zimroz, ``Rolling bearing diagnosing method based on Empirical Mode Decomposition of machine vibration signal'', \emph{Appl. Accoustics}, vol 77, pp. 195-203, 2014.

\bibitem{Rehman15} U. Abdullah, N. Rehman, M. Khan, and D. P. Mandic, ``A multivariate-EMD based approach to Pan-sharpening'', \emph{IEEE Trans Geosci Remote Sens}, vol.~53, no. 7, pp.~3974-3984,~2015.

\bibitem{Rehman13} D. P. Mandic, N. Rehman, Z. Wu, N. Huang, ``Empirical Mode Decomposition-Based Time-Frequency Analysis of Multivariate Signals: Power of Adaptive Data Analysis,'' \emph{IEEE Signal Processing Mag.}, vol. 30, no. 6, pp. 74-86, 2013.

\bibitem{Daub14} H.-T. Wu , S. S. Hseu, M. Y. Bien, Y. R. Kou, I. Daubechies, ``Evaluating physiological dynamics via synchrosqueezing: prediction of ventilator weaning,'' \emph{IEEE Trans Biomed Eng.}, vol 61, pp. 736-744, 2014.

%Rehman15N. Rehman, S. Ehsan, U. Abdullah, M. J. Akhtar, K. M. Maier, and D. P. Mandic, ``Multi-Scale Pixel based Image Fusion using Multivariate EMD'', \emph{Sensors}, vol.~20, pp.~2-27,~2015.

 %D.~P.~Mandic, N.~Rehman, and N.~Huang, ``Empirical Mode Decomposition-Based Time-Frequency Analysis of Multivariate Signals: The Power of Adaptive Data Analysis'', \emph{IEEE Signal Processing Magazine}, vol.~30, no.~6, pp.~74-86,~2013.


\bibitem{Takeda11} N. Takeda and K. Maemura, ``Circadian clock and cardiovascular disease,'' \emph{J. Cardiol.}, vol. 57, pp. 249-256, 2011.

\bibitem{Wang10} X. Wang, ``Neurophysiological and computational principles of cortical rhythms in cognition,'' \emph{Physiol. Rev.}, vol. 90, pp. 1195-1268, 2010.

\bibitem{Lin14}Y. T. Lin, H. -T. Wu, J. Tsao, H. W. Yien, S. S. Hseu, ``Time-varying spectral analysis revealing differential effects of sevoflurane anaesthesia: non-rhythmic-to-rhythmic ratio,'' \emph{Acta. Anaesthesiol. Scand.}, vol. 58, pp. 157–167, 2014.

\bibitem{Baudin14} F. Baudin, H. -T. Wu, A. Bordessoule, J. Beck, P. Jouvet, M. Frasch, G. Emeriaud, ``Impact of ventilatory modes on the breathing variability in mechanically ventilated infants'', \emph{Front. Pediatr. Sect. Neonatol.} vol. 2, pp. 132, 2014.


\bibitem{Mall11} S. Mallat, \emph{A Wavelet Tour of Signal Processing}. San Diego, CA: Academic Press, 2009.

\bibitem{Gabor46}  D. Gabor, ``Theory of Communication part 1: The analysis of information,'' \emph{Proc. Inst. Elect. Eng. III, vol. 93}, pp. 429-441, 1946.



\bibitem{Daub90}  I. Daubechies, ``The wavelet transform, time-frequency localization and signal analysis,'' \emph{IEEE Trans. Inform. Theory}, vol. 36, pp. 961-1005, 1990.

\bibitem{Daub92} I. Daubechies, \emph{Ten Lectures on Wavelets}. Philadelphia: SIAM, 1992.

\bibitem{Hlawatsch92} F. Hlawatsch and G. F. Boudreaux-Bartels, ``Linear and quadratic time frequency signal representations,'' \emph{IEEE Signal Process. Mag.}, vol. 9, no. 2, pp. 21–67, 1992.

\bibitem{Stan94} L. J. Stankovic,  ``A method for time–frequency signal analysis,'' \emph{IEEE Trans. Signal Process.}, vol. 42, pp. 225-229, 1994.

\bibitem{Auger95}F. Auger and P. Flandrin, ``Improving the readability of time-frequency and time-scale representations by the reassignment method,'' \emph{IEEE Trans. Signal Process.}, vol. 43, no. 5, pp. 1068–1089, 1995.

\bibitem{Daub96} I. Daubechies and S. Maes, ``A nonlinear squeezing of the continuous wavelet transform based on auditory nerve models,'' \emph{Wavelets Med. Biol.}, Boca Raton, FL, USA: CRC Press, 1996, pp. 527–546.

\bibitem{Auger12} F. Auger, E. Chassande-Mottin, and P. Flandrin, ``Making reassignment adjustable: The Levenberg-Marquardt approach,'' in \emph{Proc. IEEE ICASSP}, Kyoto, pp. 3889–3892, 2012.

\bibitem{Stan99} I. Djurovic and L. J. Stankovic, ``Time-frequency representation based on the reassigned S-method,'' \emph{Signal Process.}, vol. 77, no. 1, pp. 115–120, 1999.

\bibitem{Kodera76} K. Kodera, C. De Villedary, R. Gendrin, A new method for the numerical analysis of nonstationary signals,'' \emph{Phys. Earth. Plan. Int.}, vol. 12, pp. 142-150, 1976.

%---------------- Recent Variants of linear

\bibitem{Katkovnik98} V. Katkovnik, L. Stankovic, ``Instantaneous Frequency Estimation using the Wigner Distribution with Varying and Data-Driven Window Length,'' \emph{IEEE Trans. Signal Process.}, vol. 46, no. 9, pp. 2315-2325, 1998.

\bibitem{Abdoush19} Y. Abdoush, G. Pojani, G. E. Corazza,``Adaptive Instantaneous Frequency Estimation of Multicomponent Signals Based on Linear Time–Frequency Transforms,'' \emph{IEEE Trans. Signal Process.}, vol. 67, no. 12, pp. 3100–3112, 2019.

%\bibitem{Lia19} L. Lia, H. Cai, Q. Jiang, H. Ji, ``An empirical signal separation algorithm for multicomponent signals based on linear time-frequency analysis,'' \emph{Mech. Syst. Signal Process.}, vol. 121, pp. 791-809, 2019.

\bibitem{Xie12} H. Xie, J. Lin, Y. Lei, Y. Liao, ``Fast-varying AM–FM components extraction based on an adaptive STFT,'' \emph{Signal Process.}, vol. 22, pp. 664-670, 2012.

\bibitem{Olhede04} S. Olhede, A. T. Walden, ``The Hilbert spectrum via wavelet projections,'' \emph{Proc. Roy. Soc. London A}, vol. 460, pp. 955–975, 2003.

\bibitem{Gilles13} J. Gilles, ``Empirical Wavelet Transform,'' \emph{IEEE Trans. Signal Process.}, vol. 61, no. 16, pp. 3999-4010, 2013.

\bibitem{Almeida94} L. B. Almeida, ``The fractional Fourier transform and time-frequency representations,'' \emph{IEEE Trans. Signal Process.}, vol. 42, no. 11, pp. 3084-3091, 1994.

\bibitem{Stan03} L. Stankovic, T. Alieva, M. J. Bastiaans, ``Time–frequency signal analysis based on the windowed fractional Fourier transform,'' \emph{Signal Process.}, vol. 83, pp. 2459-2468, 2003.

\bibitem{FFT20} J. Shi, J. Zheng, X. Liu, W. Xiang; Q. Zhang, ``Novel Short-Time Fractional Fourier Transform: Theory, Implementation, and Applications,'' \emph{IEEE Trans. Signal Process.}, vol. 68, no. 12, pp. 3280–3295, 2020.

\bibitem{SLCT18} Y. Sun, B. Li, ``Sliding Discrete Linear Canonical Transform,'' \emph{IEEE Trans. Signal Process.}, vol. 68, no. 12, pp. 4553–4563, 2018.

\bibitem{Fland12} P. Flandrin and P. Borgnat, ``Time-frequency energy distributions meet compressed sensing,'' \emph{IEEE Trans. Signal Process.}, vol. 58, no. 6, pp. 2974-2982, 2010.

\bibitem{Stan13} L. Stanković, I. Orović, S. Stanković and M. Amin, ``Compressive Sensing Based Separation of Nonstationary and Stationary Signals Overlapping in Time-Frequency,'' \emph{IEEE Trans. Signal Process.}, vol. 61, no. 18, pp. 4562-4572, 2013.

\bibitem{Daniele13} D. Angelosante, G. B. Giannakis, N. D. Sidiropuolos, ``Sparse Parametric Models for Robust Nonstationary Signal Analysis,'' \emph{IEEE Signal Processing Mag.}, vol. 30, no. 6, pp. 64-73, 2013.

\bibitem{Balazs13} P. Balazs, M. Dorfler, M. Kowalski, B. Torresani, ``Adapted and Adaptive Linear Time-Frequency Representation,'' \emph{IEEE Signal Processing Mag.}, vol. 30, no. 6, pp. 20-31, 2013.

%\bibitem{Li19} L. Li and H. Cai, Q. Jiang and H. Ji, ``An empirical signal separation algorithm for multicomponent signals based on linear time-frequency analysis,'' \emph{Mechanical Systems and Signal Processing}, vol. 121, no. 4, pp. 791-809, 2019.

\bibitem{Huang09} N. E. Huang, Z. Wu, S. R. Long, K. C. Arnold, X. Chen and K. Blank, ``On Instantaneous Frequency'', \emph{Adv. Adapt. Data Anal.}, vol. 1, pp. 177-229, 2009.

\bibitem{Meignen07} S. Meignen and V. Perrier, ``A new formulation for empirical mode decomposition based on constraint optimization'', \textit{IEEE Signal Processing Letters}, vol. 14, pp. 932-935, 2007.

\bibitem{Pustelnik14} N. Pustelnik, P. Borgnat and P. Flandrin, ``Empirical mode decomposition revisited by multicomponent non-smooth convex optimization,'' \textit{Signal Processing}, vol. 102, pp. 313-331, 2014.

\bibitem{Lin09} L. Lin, Y. Wang, H. Zhou, ``Iterative filtering as an alternative algorithm for empirical mode decomposition,'' \emph{Adv. Adapt. Data Anal.}, Vol 1, no. 4, pp. 543–560, 2009.

\bibitem{Cicone16} C. Cicone, J. Liu, H. Zhou, ``Adaptive local iterative filtering for signal decomposition and instantaneous frequency analysis,'' \emph{Appl. Comput. Harmon. Anal.}, vol. 30, no. 2, pp. 243–261, 2011.

\bibitem{Hou11} T. Y. Hou, Z. Shi, ``Adaptive Data Analysis via Sparse Time-Frequency Representation,'' \emph{Adv. Adapt. Data Anal.}, vol. 3, no. 1, pp. 1-28, 2011.

\bibitem{Hou16} T. Y. Hou, Z. Shi, ``Sparse time-frequency decomposition based on dictionary adaptation,'' \emph{Phil. Trans. R. Soc. A}, vol. 374, pp. 20150192, 2016.

\bibitem{Wu09} Z. Wu and N. E. Huang, ``Ensemble empirical mode decomposition: a noise-assisted data analysis method,'' \emph{Adv. Adapt. Data Anal.}, vol. 1, no. 1, pp. 1-41, 2009.

\bibitem{Rehman13-AADA} N. Rehman, C. Park, N. E. Huang, and D. P. Mandic, ``EMD via MEMD multivariate noise-aided computation of standard EMD,'' \emph{Adv. Adapt. Data Anal.}, vol. 5, no. 2, pp. 1–25, 2013.

\bibitem{Lang20} X. Lang, N. Rehman, Y. Zhang, L. Xie, H. Su, ``Median ensemble empirical mode decomposition,'' \emph{Signal Process.}, vol. 176, 2020.


%

%\bibitem{Rilling08} G. Rilling and P. Flandrin, ``One or two frequencies? The Empirical Mode Decomposition answers,'' \emph{IEEE Trans. Signal Processing}, vol. 56, no. 1, pp. 85–95, 2008.

%------------------------- SST
\bibitem{SST_SPM13} F. Auger, P. Flandrin, Y. Lin, S. McLaughlin, S. Meignen, T. Oberlin, H. Wu, ``Time-Frequency Reassignment and Synchrosqueezing,'' \emph{IEEE Signal Process. Mag.}, vol. , pp. 32-41, 2013.


\bibitem{Thakur11} J. Thakur and H.-T. Wu, ``Synchrosqueezing based recovery of instantaneous frequency from nonuniform samples,'' \emph{SIAM J. Math. Anal.}, vol. 43, no. 5, pp. 2078–2095, 2011.

\bibitem{Thakur13} G. Thakur, E. Brevdo, N. S. Fuckar, and H.-T. Wu, ``The synchrosqueezing algorithm for time-varying spectral analysis: Robustness properties and new paleoclimate applications,'' \emph{Signal Process.}, vol. 93, no. 5, pp. 1079–1094, 2013.

\bibitem{Huang16} Z. Huang, J. Zhang, T. Zhao, and Y. Sun, ``Synchrosqueezing S-Transform and its Application in Seismic Spectral Decomposition,'' \emph{IEEE Trans. GeoSci. Remote Sens.}, vol. 54, no. 2, pp. 817-825, 2016.

\bibitem{daub15} I. Daubechies, Y. Wang, H. Wu, ``ConceFT: Concentration of frequency and time via a multitapered synchrosqueezed transform,'' \emph{Phil. Trans. R. Soc. A}, vol. 374, pp. 20150193, 2016.

\bibitem{Oberlin15} T. Oberlin, S. Meignen, and V. Perrier, ``Second-Order Synchrosqueezing Transform or Invertible Reassignment? Towards Ideal Time-Frequency Representations,'' \emph{IEEE Trans. Signal Process.}, vol. 63, no. 5, pp. 1335–1344, 2015.

\bibitem{Bahera18} R. Bahera, S. Meignen, T. Oberlin, ``Theoretical analysis of the second-order synchrosqueezing transform,'' \emph{Appl. Comput. Harmon. Anal.}, vol. 35, no. 2, pp. 379-404, 2018.

\bibitem{Pham17} D. Pham, S. Meignen, ``High-Order Synchrosqueezing Transform for Multicomponent Signals Analysis -- With an Application to Gravitational-Wave Signal,''  \emph{IEEE Trans. Signal Process.}, vol. 62, no. 12, pp. 3168-3178, 2017.

\bibitem{Yang18} H. Z. Yang, ``Statistical analysis of synchrosqueezed transforms,'' \emph{Appl. Comput. Harmon. Anal.}, vol. 45, no. 3, pp. 526-550, 2018.

\bibitem{Chui16} C. K. Chui and H. N. Mhaskar, ``Signal decomposition and analysis via extraction of frequencies,'' \emph{Appl. Comput. Harmon. Anal.}, vol. 40, no. 1, pp. 97-136, 2016.

\bibitem{Li20} L. Li, C. K. Chui, Q. Jian``Direct Signal Separation Via Extraction of Local Frequencies with Adaptive Time-Varying Parameters'', \emph{arXiv:2010.01866}, 2020.

\bibitem{Meignen17} S. Meignen, D. Pham, S. McLaughlin, ``On Demodulation, Ridge Detection, and Synchrosqueezing for Multicomponent Signals,'' \emph{IEEE Trans. Signal Process.}, vol. 65, no. 8, pp. 2093-2103, 2017.

\bibitem{Laurent20} N. Laurent, S. Meignen, ``A Novel Approach for Ridge Detection and Mode Retrieval of Multicomponent Signals Based on STFT,'' \emph{arXiv:2009.13123v1}, 2020.

%\bibitem{Jiang17} Q. Jiang and B. W. Suter, ``Instantaneous frequency estimation based on synchrosqueezing wavelet transform,'' \emph{Signal Process.}, vol. 138, pp.167-181, 2017.



%----------------------------------------- VMD based

\bibitem{VMD14} K. Dragomiretskiy, D. Zosso, ``Variational Mode Decomposition'',  \emph{IEEE Trans. Signal Processing}, vol. 62, no. 3, pp. 531-544, 2014.

\bibitem{NCMD18} S. Chen, X. Dong, Z. Peng, W. Zhang, G. Meng, ``Nonlinear Chirp Mode Decomposition'',  \emph{IEEE Trans. Signal Processing}, vol. 65, no. 22, pp. 6024-6037, 2017.

%---------------------- ICA based approaches
\bibitem{Comon94} P. Comon, ``Independent Component Analysis, a new concept?,'' \emph{Signal Process.}, vol. 36, pp. 287-314, 1994.
36, pp.287-314

\bibitem{Lee99} D. D. Lee and H. S. Seung, ``Learning the parts of objects with nonnegative matrix factorization,'' \emph{Nature}, vol. 401, pp. 788–791, 1999.

\bibitem{Smaragdis14} P. Smaragdis, C. Févotte, G. J. Mysore, N. Mohammadiha, M. Hoffman, ``Static and Dynamic Source Separation Using Nonnegative Factorizations,'' \emph{IEEE Signal Processing Mag.}, vol. 32, no. 3, pp. 66-75, 2014.

\bibitem{Broomhead86} D. Broomhead and G. King, ``Extracting qualitative dynamics from experimental data,'' \emph{Physica D}, vol. 20, pp. 217–236, 1986.

\bibitem{Schmid10} P. J. Schmid, ``Dynamic mode decomposition of numerical and experimental data,'' \emph{J. Fluid Mech.}, vol. 656, pp. 5–28, 2010.

\bibitem{Fland18} J. Harmouche, D. Fourer, F. Auger, P. Borgnat, P. Flandrin, ``The Sliding Singular Spectrum Analysis: a Data-Driven Non-Stationary Signal Decomposition Tool,'' \emph{IEEE Trans. Signal Process.}, vol. 66, no. 1, pp. 251-263, 2018.

\bibitem{LTFRS18} C. Févotte, M. Kowalski, ``Estimation With Low-Rank Time–Frequency Synthesis Models,''  \emph{IEEE Trans. Signal Process.}, vol. 66, no. 15, pp. 4121-4132, 2018.

%\bibitem{Amin98} A. Belouchrani, M. G. Amin, ``Blind Source Separation Based on Time–Frequency Signal Representations,'' \emph{IEEE Trans. Signal Process.}, vol. 46, no. 11, pp. 2888-2897, 2017.

%------------------------ Multivariate
\bibitem{Rehman09} N.~Rehman and D.~P.~Mandic, ``Multivariate Empirical Mode Decomposition,'' \emph{Proceedings of the Royal Society A}, vol.~466, no.~2117, pp.~1291-1302,~2010.

\bibitem{Rehman10} N. Rehman and D. P. Mandic, ``Empirical Mode Decomposition for Trivariate Signals,'' \emph{IEEE Trans. Signal Processing}, vol. 58, no. 3, pp. 1059-1068, 2010.

\bibitem{Rehman11} N. Rehman and D. P. Mandic, ``Filter Bank Property of Multivariate Empirical Mode Decomposition'', \emph{IEEE Trans. Signal Processing}, vol. 59, no. 5, pp. 2421-2426, 2011.




%
\bibitem{Cicone19} A. Cicone, ``Multivariate Fast Iterative Filtering for the decomposition of nonstationary signals,'' \emph{arXiv: 1902.04860}, 2019.

\bibitem{Rehman19} N. Rehman and H. Aftab, ``Multivariate Variational Mode Decomposition,'' \emph{IEEE Trans. Signal Process.}, vol. 67, no. 3, pp. 6039-6052, 2019.

\bibitem{Chen20} Q. Chen, L. Xie, H. Su, ``Multivariate nonlinear chirp mode decomposition,'' \emph{Signal Process.}, vol. 176, 2020.

\bibitem{Ali15} A. Ahrabian, D. Looney, L. Stankovic, D. P. Mandic, ``Synchrosqueezing-based time-frequency analysis of multivariate data,'' \emph{Signal Process.}, vol. 106, pp. 331-341, 2015.

\bibitem{MEWT18} O. Singh, R. K. Sunkaria, ``An empirical wavelet transform based approach for multivariate data processing application to cardiovascular physiological signals,'' \emph{Bio Alg. Med. Syst.}, vol. 14, no. 4, 2018.

\bibitem{Jain20} S. Jain, R. Panda, R. K. Tripathy, ``Multivariate Sliding-Mode Singular Spectrum Analysis for the Decomposition of Multisensor Time Series,'' \emph{IEEE Sens. Lett.}, vol. 4, no. 6, pp. 2475-147, 2020.

\bibitem{Stan20} L. Stankovic, M. Brajovi, M. Dakovi, D. P. Mandic, ``On the decomposition of multichannel nonstationary multicomponent signals,'' \emph{Signal Process.}, vol. 167, pp. 107261, 2020.

%----------------------- Nonconvex
\bibitem{Boyd04} S. Boyd, L. Vandenberghe, \emph{Convex Optimization}. New York, NY: Cambridge University Press, 2004.

\bibitem{Candes10}E. Candès and T. Tao, ``The power of convex relaxation: Near-optimal matrix completion,'' \emph{IEEE Trans. Inf. Theory}, vol. 56, no. 5, pp. 2053–2080, 2010.

\bibitem{Candes11} E. J. Candès, X. Li, Y. Ma, and J. Wright, ``Robust principal component analysis?,'' \emph{J. ACM}, vol. 58, no. 3, pp. 11:1–11:37, 2011.

\bibitem{Chandrasekaran11} V. Chandrasekaran, S. Sanghavi, P. Parrilo, and A. Willsky, ``Rank sparsity incoherence for matrix decomposition,'' \emph{SIAM J. Optim.}, vol. 21, no. 2, pp. 572–596, 2011.

\bibitem{Ahmad14} A. Ahmed, B. Recht, and J. Romberg, ``Blind deconvolution using convex programming,'' \emph{IEEE Trans. Inf. Theory}, vol. 60, no. 3, pp. 1711–1732, 2014.

\bibitem{Chi18} Y. Chen and Y. Chi, ``Harnessing structures in big data via guaranteed low-rank matrix estimation: Recent theory and fast algorithms via convex and nonconvex optimization,'' \emph{IEEE Signal Process. Mag.}, vol. 35, no. 4, pp. 14–31, Jul. 2018.

\bibitem{Jain17} P. Jain and P. Kar, ``Non-convex optimization for machine learning,'' \emph{Foundations Trends Machine Learn.}, vol. 10, no. 3–4, pp. 142–336, 2017.

\bibitem{Chi19} Y. Chi, Y. M, Lu, Y. Chen, ``Nonconvex Optimization Meets Low-Rank Matrix Factorization: An Overview,'' \emph{IEEE Trans. Signal Proces.}, vol. 67, no. 20, pp. 5239-5269, 2019.

\bibitem{cond19} W. Zhang, D. Yang, H. Wang, ``Data-Driven Methods for Predictive Maintenance of Industrial Equipment:
A Survey,'' \emph{IEEE Syst. J.}, vol. 13, pp. 2213–2227, 2019.


\bibitem{Morse20} K. E. Morse, S. C. Bagley and N. H. Shah,``Estimate the hidden deployment cost of predictive models to improve patient care,'' \emph{Nat. Med.}, vol. 26, pp. 18–19, 2020.

\bibitem{Mandic17} V. Goverdovsky, W. von Rosenberg, T. Nakamura et al. ``Hearables: Multimodal physiological in-ear sensing,'' \emph{Sci Rep}, vol. 7, no. 6948, 2017.

\bibitem{Sharma20} P. Sharma, X. Hui, J. Zhou et al. ``Wearable radio-frequency sensing of respiratory rate, respiratory volume, and heart rate,'' \emph{Digit. Med.}, vol. 3, no. 98, 2020.

\bibitem{Vaswani20} N. Vaswani, ``Nonconvex Structured Phase Retrieval: A Focus on Provably Correct Approaches,'' \emph{IEEE Signal Processing Mag.}, vol. 37, no. 5, pp. 67-77, 2020.

\bibitem{Looney12} D. Looney, P. Kidmose, C. Park, M. Ungstrup, M. L. Rank, K. Rosenkranz and D. P. Mandic, ``The In-the-Ear Recording Concept: User-Centered and Wearable Brain Monitoring,'' \emph{IEEE Pulse}, vol. 3, no. 6, pp. 32-42, 2012.
\bibitem{Aimoni18} C. Aimoni, L. Crema, S. Savini, et al. ``Hearing threshold estimation by auditory steady state responses (ASSR) in children'', \emph{Acta Otorhinolaryngol Ital.}, vol. 38, pp. 361-368, 2018.
\bibitem{Wu20} H-T Wu, ``Current state of nonlinear-type time–frequency analysis and applications to high-frequency biomedical signals,'' \emph{Current Opinion in Systems Biology}, vol. 23, pp. 8-11, 2020.
\bibitem{Zhang17} X. S. Zhang and F. Wang, ``Signal Processing for Finance, Economics, and Marketing: Concepts, framework, and big data applications,'' \emph{IEEE Signal Process. Mag.}, vol. 34, no. 3, pp. 14-35, 2017.
\bibitem{Takeuchi20} D. Takeuchi, K. Yatabe, Y. Koizumi, Y. Oikawa, N. Harada,``Invertible DNN-based nonlinear time-frequency transform for speech enhancement,'' \emph{arXiv:1911.10764v2}, 2020.
\bibitem{Wong18} L. Wong, Y. Chen, Q. Wang, V. Kuehnel, ``Efficacy of a Hearing Aid Noise Reduction Function,'' \emph{Trends Hear.}, vol. 22, 2018.


% ------------------------ Ear EEG, Hyperscanning

%\bibitem{Looney12} D. Looney, P. Kidmose, C. Park, M. Ungstrup, M. L. Rank, K. Rosenkranz, D. Mandic, ``The In-the-Ear Recording Concept: User-Centered and Wearable Brain Monitoring,'' \emph{IEEE Pulse}, vol. 3, no. 6, pp. 32-42, 2012.

%\bibitem{Kidmose13} P. Kidmose, D. Looney, M. Ungstrup, M. L. Rank and D. P. Mandic, ``A Study of Evoked Potentials From Ear-EEG,'' \emph{IEEE Trans. Biomedical Eng.}, vol. 60, no. 10, pp. 2824-2830, 2013.

%\bibitem{Kappel19} S. L. Kappel, M. L. Rank, H. O. Toft, M. Andersen and P. Kidmose, ``Dry-Contact Electrode Ear-EEG,'' \emph{IEEE Trans. Biomedical Eng.}, vol. 66, no. 1, pp. 150-158, 2019.

%

%\bibitem{Aimoni18} C. Aimoni, L. Crema, S. Savini, et al. ``Hearing threshold estimation by auditory steady state responses (ASSR) in children'', \emph{Acta Otorhinolaryngol Ital.}, vol. 38, pp. 361-368, 2018.



%\bibitem{Rehman13} D. P. Mandic, N. Rehman, Z. Wu, N. E. Huang, ``Empirical Mode Decomposition-Based Time-Frequency Analysis of Multivariate Signals: The Power of Adaptive Data Analysis'', \emph{IEEE Signal Process. Mag.}, vol. 30, pp. 74-86, 2013.

\bibitem{ChenML19} J. Chen and X. Ran, ``Deep learning with edge computing: A review,'' \emph{Proc. IEEE}, vol 107, pp. 1655-1674, 2019.

\bibitem{Yonina20} N. Shlezinger, J. Whang, Y. C. Eldar and A. G. Dimakis, ``Model based deep learning'', \emph{arXiv:2012.08405v1}, 2020.

%--------------- Basin of att

\bibitem{Jain13} P. Jain, P. Netrapalli, and S. Sanghavi, ``Low-rank matrix completion using alternating minimization,'' \emph{in Proc. 45th Annu. ACM Symp. Theory Comput.}, ACM, 2013, pp. 665–674.

\bibitem{Jain16} Y. Cherapanamjeri, K. Gupta, P. Jain, ``Nearly optimal robust matrix completion,'' \emph{in Proc. Int. Conf. Machine Learning.}, 2016.

\bibitem{Jain14} P. Netrapalli, U. N. Niranjan, S. Sanghavi, A. Anandkumar and P. Jain, ``Nonconvex robust PCA,'' \emph{in Proc. Conf. Neural Inf. Process. Systems}, 2014, pp. 1107-1115.

\bibitem{Keshavan10} R. H. Keshavan, A. Montanari, and S. Oh, ``Matrix completion from a few entries,'' \emph{IEEE Trans. Inf. Theory}, vol. 56, no. 6, pp. 2980–2998, 2010.

\bibitem{Chen15} Y. Chen, M. J. Wainwright, ``Fast low-rank estimation by projected gradient descent: General statistical and algorithmic guarantees,'' \emph{arXiv:1509.03025}, 2015.

\bibitem{Candes15} E. Candès, X. Li, and M. Soltanolkotabi, ``Phase retrieval via Wirtinger flow: Theory and algorithms,'' \emph{IEEE Trans. Inf. Theory}, vol. 61, no. 4, pp. 1985–2007, 2015.

\bibitem{Zhang16} H. Zhang, Y. Chi, Y. Liang, ``Provable non-convex phase retrieval with outliers: Median truncated Wirtinger flow,'' \emph{in Proc. Int. Conf. Mach. Learn.}, 2016, pp. 1022–1031.

%------------------ no spurious minima

\bibitem{Ge16} R. Ge, J. D. Lee, T. Ma, ``Matrix completion has no spurious local minimum,'' \emph{in Proc. Adv. Neural Inf. Process. Syst.}, 2016, pp. 2973–2981.

\bibitem{Sun16} R. Sun, Z.-Q. Luo, ``Guaranteed matrix completion via non-convex factorization,'' \emph{IEEE Trans. Inf. Theory}, vol. 62, no. 11, pp. 6535–6579, 2016.

\bibitem{Tu16} S. Tu, R. Boczar, M. Simchowitz, M. Soltanolkotabi, B. Recht, ``Low rank solutions of linear matrix equations via Procrustes flow,'' \emph{in Proc. Int. Conf. Mach. Learn.}, 2016, pp. 964–973.

\bibitem{Bhojanapalli16} S. Bhojanapalli, B. Neyshabur, N. Srebro, ``Global optimality of local search for low rank matrix recovery,'' \emph{in Proc. Adv. Neural Inf. Process. Syst.}, 2016, pp. 3873–3881.

%\bibitem{Chen17} Y. Chen, E. Candès, ``Solving random quadratic systems of equations is nearly as easy as solving linear systems,'' \emph{Commun. Pure Appl. Math.}, vol. 70, no. 5, pp. 822–883, 2017.

\bibitem{Ge15} R. Ge, F. Huang, C. Jin, Y.Yuan, ``Escaping from saddle points-online stochastic gradient for tensor decomposition,'' \emph{in Proc. Conf. Learn. Theory}, pp. 797–842, 2015.

%-------------
%\bibitem{Ozerov10} A. Ozerov and C. Fevotte, ``Multichannel nonnegative matrix factorization in convolutive mixtures for audio source separation,'' \emph{IEEE Trans. Audio Speech Lang. Process.}, vol. 18, no. 3, pp. 550–563, 2010.

\bibitem{Fevotte11} C. Fevotte and J. Idier, ``Algorithms for nonnegative matrix factorization with the $\beta$-divergence,'' \emph{Neural Comput.}, vol. 23, no. 9, pp. 2421–2456, 2011.

\bibitem{Emiya18} V. Emiya, R. Hamon and C. Chaux, ``Being Low-Rank in the Time-Frequency Plane,'' \emph{in Proceedings IEEE (ICASSP)}, Calgary, pp. 4659-4663, 2018.

%\bibitem{Rehman13-AADA} N. Rehman, C. Park, N. E. Huang, and D. Mandic, ``EMD via MEMD multivariate noise-aided computation of standard EMD,'' \emph{Adv. Adapt. Data Anal.}, vol. 5, no. 2, pp. 1–25, 2013.

%\bibitem{Rehman11} N. Rehman and D. Mandic, ``Filter Bank Property of Multivariate Empirical Mode Decomposition'', \emph{IEEE Trans. Signal Processing}, vol. 59, no. 5, pp. 2421-2426, 2011.

%--------------------------???
\bibitem{Boyd11} S. Boyd, N. Parikh, E. Chu, B. Peleato, and J. Eckstein, ``Distributed Optimization and Statistical Learning via the Alternating Direction Method of Multipliers,'' \emph{Found. Trends Mach. Learn.}, vol. 3, pp. 1-22, 2011.

\bibitem{Chen19} Y. Chen, Y. Chi, J. Fan, and C. Ma, ``Gradient descent with random initialization: fast global convergence for nonconvex phase retrieval,'' \emph{Math. Program.}, vol. 176, no. 1-2, pp. 5-37, 2019.

\bibitem{NGD2} Z. Allen-Zhu, ``Natasha 2: Faster non-convex optimization than SGD,'' \emph{in Proc. Neural Inf. Process. Syst.}, 2018, pp. 2675–2686.

\bibitem{NGD3} Y. Xu, J. Rong, and T. Yang, ``First-order stochastic algorithms for escaping from saddle points in almost linear time,'' \emph{in Proc. Adv. Neural Inf. Process. Syst.}, 2018, pp. 5530–5540.

\bibitem{NGD4} Z. Allen-Zhu and Y. Li, ``Neon2: Finding local minima via first-order oracles,'' \emph{in Proc. Neural Inf. Process. Syst.}, 2018, pp. 3716–3726.
    
    \bibitem{Jin17} C. Jin, R. Ge, P. Netrapalli, S. M. Kakade, and M. I. Jordan, ``How to escaping saddle points efficiently,'' \emph{in Proc. Int. Conf. Machine Learn.}, 2017, pp. 1724-1732.

%--------------------- Denoising

%\bibitem{Donoho95} D. Donoho, ``De-noising by soft-thresholding,'' \emph{IEEE Trans. Inf. Theory}, vol. 41, no. 3, pp. 613–627, 1995.

%\bibitem{Rehman17} N. Rehman, Z. Abbas, A. Asif, A. Javed, K. Naveed and D. P. Mandic,   ``Translation invariant multi-scale signal denoising based on goodness-of-fit tests,'' \emph{Signal Process.}, vol. 121, pp. 230-244, 2017.

\bibitem {Hao17} H. Hao, H.L. Wang and N. Rehman, ``A joint framework for multivariate signal denoising using multivariate empirical mode decomposition,'' \emph{Signal Process.}, vol. 135, pp. 263-273, 2017.

\bibitem{Rehman19SPL} N. Rehman, B. Khan and K. Naveed ``Multivariate Signal Denoising using Mahalanobis Distance,'' \emph{IEEE Signal Processing Lett.}, vol. 26, pp. 1408-1412, 2019.

\bibitem{Rehman20} K. Naveed and N. Rehman, ``Wavelet based multivariate signal denoising using Mahalanobis distance and EDF statistics,'' \emph{IEEE Trans. Signal Process.}, vol. 68, pp. 5997-6010, 2020.

\bibitem{Park12} C. Park, D. Looney, P. Kidmose, M. Ungstrp, D. P. Mandic, ``Time-frequency analysis of EEG asymmetry using bivariate empirical mode decomposition,'' \emph{IEEE Trans. Neural Syst. Rehabilitation Eng.}, vol. 19, no. 4, pp. 366-373, 2011.

\bibitem{Hyperscanning14} F. Babilonia, L. Astolfia, ``Social neuroscience and hyperscanning techniques: Past, present and future,'' \emph{Neuroscience  Biobehavioral Rev.}, vol . 44, pp. 76-93, 2014.

\bibitem{Parra19} L. C. Parra, S. Haufe, J. P. Dmochowski, ``Correlated Components Analysis -- Extracting Reliable Dimensions in Multivariate Data,'' \emph{Neurons Behav. Data Anal. Theory (NBDT)}, arXiv:1801.08881, 2019.

\end{thebibliography}



==> Naveed_References <==
%\footnotesize
\begin{thebibliography}{200} % 100 is a random guess of the total number of

\bibitem{Flandrin18} P. Flandrin, \emph{Explorations in Time-Frequency Analysis}. New York, NY: Cambridge University Press, 2018.

\bibitem{SPM20} A. M. -C. So, P. Jain, W. -K. Ma and G. Scutari, ``Nonconvex Optimization for Signal Processing and Machine Learning [From the Guest Editors],'' \emph{IEEE Signal Process. Mag.}, vol. 37, no. 5, pp. 15-17, 2020.

%
\bibitem{Cohen95} L. Cohen, \emph{Time-Frequency Analysis: Theory and Applications}. Englewood Cliffs, NJ: Prentice Hall, 1995.




%\bibitem{Fland99} P. Flandrin, \emph{Time-Frequency/Time-Scale analysis}. San Diego, CA: Academic Press, 1999.



%\bibitem{Ville48} J. Ville, ``Théorie et Applications de la Notion de Signal Analytique,'' \emph{Câbles et Transmission}, vol. 2, pp. 61–74, 1948.

\bibitem{Huang98} N. E. Huang, Z. Shen, S. R. Long, Wu, M. L., H. H. Shih, Q. Zheng, N. C. Yen, C. C. Tung, and H. H. Liu, ``The Empirical Mode Decomposition and Hilbert spectrum for nonlinear and non-stationary time series analysis,'' \emph{Proc. R. Soc. Lond. A, Math. Phys. Sci.}, vol. 454, no. 1971, pp. 903–995, 1998.

\bibitem{Daub11} I. Daubechies, J. Lu, and H. T. Wu, ``Synchrosqueezed wavelet transforms: An Empirical Mode Decomposition-like tool,'' \emph{Appl. Comput. Harmon. Anal.}, vol. 41, pp. 384-411, 2016.

\bibitem{Maragos01} A. Potamianos and P. Maragos,  ``Time-Frequency Distributions for Automatic Speech Recognition,'' \emph{IEEE Trans. Speech Audio Process.}, vol. 9, pp. 196-200, 2001.

\bibitem{Mallat08} G. Yu, S. Mallat, and E. Bacry, ``Audio denoising by time-frequency block thresholding,'' \emph{IEEE Trans. Signal Process.}, vol. 56, pp. 1830-1839. 2008.

%\bibitem{Necciari13} T. Necciari, P. Balazs, N. Holighaus, and P. Soendergaard,  ``The ERBlet transform: An auditory-based time-frequency representation with perfect reconstruction,'' \emph{Proc. IEEE Int. Conf. Acoustics, Speech, and Signal Processing (ICASSP)}, 2013.

\bibitem{Matz13} G. Matz, H. Bolcskei and F. Hlawatsch, ``Time-Frequency Foundations of Communications: Concepts and Tools,'' \emph{IEEE Signal Process. Mag.}, vol. 30, pp. 87-96, 2013.

\bibitem{Park13} C. Park, D. Looney, N. Rehman and D. P. Mandic, ``Motor imagery signal classification using multivariate empirical mode decomposition'', \emph{IEEE Trans. Neural Syst. Rehabilitation Eng.}, vol. 21, pp. 10-22, 2013.

\bibitem{Saleem19} S. Saleem, S. S. Naqvi, T. Manzoor, A. Saeed, N. Rehman, J. Mirza, ``A strategy for classification of vaginal vs. cesarean section delivery: bivariate empirical mode decomposition of cardiotocographic recordings,'' \emph{Front. Physiol.}, vol. 10, pp. 246, 2019.

\bibitem{Dybala14} J. Dybala and R. Zimroz, ``Rolling bearing diagnosing method based on Empirical Mode Decomposition of machine vibration signal'', \emph{Appl. Accoustics}, vol 77, pp. 195-203, 2014.

\bibitem{Rehman15} U. Abdullah, N. Rehman, M. Khan, and D. P. Mandic, ``A multivariate-EMD based approach to Pan-sharpening'', \emph{IEEE Trans Geosci Remote Sens}, vol.~53, no. 7, pp.~3974-3984,~2015.

\bibitem{Rehman13} D. P. Mandic, N. Rehman, Z. Wu, N. Huang, ``Empirical Mode Decomposition-Based Time-Frequency Analysis of Multivariate Signals: Power of Adaptive Data Analysis,'' \emph{IEEE Signal Processing Mag.}, vol. 30, no. 6, pp. 74-86, 2013.

\bibitem{Daub14} H.-T. Wu , S. S. Hseu, M. Y. Bien, Y. R. Kou, I. Daubechies, ``Evaluating physiological dynamics via synchrosqueezing: prediction of ventilator weaning,'' \emph{IEEE Trans Biomed Eng.}, vol 61, pp. 736-744, 2014.

%Rehman15N. Rehman, S. Ehsan, U. Abdullah, M. J. Akhtar, K. M. Maier, and D. P. Mandic, ``Multi-Scale Pixel based Image Fusion using Multivariate EMD'', \emph{Sensors}, vol.~20, pp.~2-27,~2015.

 %D.~P.~Mandic, N.~Rehman, and N.~Huang, ``Empirical Mode Decomposition-Based Time-Frequency Analysis of Multivariate Signals: The Power of Adaptive Data Analysis'', \emph{IEEE Signal Processing Magazine}, vol.~30, no.~6, pp.~74-86,~2013.


\bibitem{Takeda11} N. Takeda and K. Maemura, ``Circadian clock and cardiovascular disease,'' \emph{J. Cardiol.}, vol. 57, pp. 249-256, 2011.

\bibitem{Wang10} X. Wang, ``Neurophysiological and computational principles of cortical rhythms in cognition,'' \emph{Physiol. Rev.}, vol. 90, pp. 1195-1268, 2010.

\bibitem{Lin14}Y. T. Lin, H. -T. Wu, J. Tsao, H. W. Yien, S. S. Hseu, ``Time-varying spectral analysis revealing differential effects of sevoflurane anaesthesia: non-rhythmic-to-rhythmic ratio,'' \emph{Acta. Anaesthesiol. Scand.}, vol. 58, pp. 157–167, 2014.

\bibitem{Baudin14} F. Baudin, H. -T. Wu, A. Bordessoule, J. Beck, P. Jouvet, M. Frasch, G. Emeriaud, ``Impact of ventilatory modes on the breathing variability in mechanically ventilated infants'', \emph{Front. Pediatr. Sect. Neonatol.} vol. 2, pp. 132, 2014.


\bibitem{Mall11} S. Mallat, \emph{A Wavelet Tour of Signal Processing}. San Diego, CA: Academic Press, 2009.

\bibitem{Gabor46}  D. Gabor, ``Theory of Communication part 1: The analysis of information,'' \emph{Proc. Inst. Elect. Eng. III, vol. 93}, pp. 429-441, 1946.



\bibitem{Daub90}  I. Daubechies, ``The wavelet transform, time-frequency localization and signal analysis,'' \emph{IEEE Trans. Inform. Theory}, vol. 36, pp. 961-1005, 1990.

\bibitem{Daub92} I. Daubechies, \emph{Ten Lectures on Wavelets}. Philadelphia: SIAM, 1992.

\bibitem{Hlawatsch92} F. Hlawatsch and G. F. Boudreaux-Bartels, ``Linear and quadratic time frequency signal representations,'' \emph{IEEE Signal Process. Mag.}, vol. 9, no. 2, pp. 21–67, 1992.

\bibitem{Stan94} L. J. Stankovic,  ``A method for time–frequency signal analysis,'' \emph{IEEE Trans. Signal Process.}, vol. 42, pp. 225-229, 1994.

\bibitem{Auger95}F. Auger and P. Flandrin, ``Improving the readability of time-frequency and time-scale representations by the reassignment method,'' \emph{IEEE Trans. Signal Process.}, vol. 43, no. 5, pp. 1068–1089, 1995.

\bibitem{Daub96} I. Daubechies and S. Maes, ``A nonlinear squeezing of the continuous wavelet transform based on auditory nerve models,'' \emph{Wavelets Med. Biol.}, Boca Raton, FL, USA: CRC Press, 1996, pp. 527–546.

\bibitem{Auger12} F. Auger, E. Chassande-Mottin, and P. Flandrin, ``Making reassignment adjustable: The Levenberg-Marquardt approach,'' in \emph{Proc. IEEE ICASSP}, Kyoto, pp. 3889–3892, 2012.

\bibitem{Stan99} I. Djurovic and L. J. Stankovic, ``Time-frequency representation based on the reassigned S-method,'' \emph{Signal Process.}, vol. 77, no. 1, pp. 115–120, 1999.

\bibitem{Kodera76} K. Kodera, C. De Villedary, R. Gendrin, A new method for the numerical analysis of nonstationary signals,'' \emph{Phys. Earth. Plan. Int.}, vol. 12, pp. 142-150, 1976.

%---------------- Recent Variants of linear

\bibitem{Katkovnik98} V. Katkovnik, L. Stankovic, ``Instantaneous Frequency Estimation using the Wigner Distribution with Varying and Data-Driven Window Length,'' \emph{IEEE Trans. Signal Process.}, vol. 46, no. 9, pp. 2315-2325, 1998.

\bibitem{Abdoush19} Y. Abdoush, G. Pojani, G. E. Corazza,``Adaptive Instantaneous Frequency Estimation of Multicomponent Signals Based on Linear Time–Frequency Transforms,'' \emph{IEEE Trans. Signal Process.}, vol. 67, no. 12, pp. 3100–3112, 2019.

%\bibitem{Lia19} L. Lia, H. Cai, Q. Jiang, H. Ji, ``An empirical signal separation algorithm for multicomponent signals based on linear time-frequency analysis,'' \emph{Mech. Syst. Signal Process.}, vol. 121, pp. 791-809, 2019.

\bibitem{Xie12} H. Xie, J. Lin, Y. Lei, Y. Liao, ``Fast-varying AM–FM components extraction based on an adaptive STFT,'' \emph{Signal Process.}, vol. 22, pp. 664-670, 2012.

\bibitem{Olhede04} S. Olhede, A. T. Walden, ``The Hilbert spectrum via wavelet projections,'' \emph{Proc. Roy. Soc. London A}, vol. 460, pp. 955–975, 2003.

\bibitem{Gilles13} J. Gilles, ``Empirical Wavelet Transform,'' \emph{IEEE Trans. Signal Process.}, vol. 61, no. 16, pp. 3999-4010, 2013.

\bibitem{Almeida94} L. B. Almeida, ``The fractional Fourier transform and time-frequency representations,'' \emph{IEEE Trans. Signal Process.}, vol. 42, no. 11, pp. 3084-3091, 1994.

\bibitem{Stan03} L. Stankovic, T. Alieva, M. J. Bastiaans, ``Time–frequency signal analysis based on the windowed fractional Fourier transform,'' \emph{Signal Process.}, vol. 83, pp. 2459-2468, 2003.

\bibitem{FFT20} J. Shi, J. Zheng, X. Liu, W. Xiang; Q. Zhang, ``Novel Short-Time Fractional Fourier Transform: Theory, Implementation, and Applications,'' \emph{IEEE Trans. Signal Process.}, vol. 68, no. 12, pp. 3280–3295, 2020.

\bibitem{SLCT18} Y. Sun, B. Li, ``Sliding Discrete Linear Canonical Transform,'' \emph{IEEE Trans. Signal Process.}, vol. 68, no. 12, pp. 4553–4563, 2018.

\bibitem{Fland12} P. Flandrin and P. Borgnat, ``Time-frequency energy distributions meet compressed sensing,'' \emph{IEEE Trans. Signal Process.}, vol. 58, no. 6, pp. 2974-2982, 2010.

\bibitem{Stan13} L. Stanković, I. Orović, S. Stanković and M. Amin, ``Compressive Sensing Based Separation of Nonstationary and Stationary Signals Overlapping in Time-Frequency,'' \emph{IEEE Trans. Signal Process.}, vol. 61, no. 18, pp. 4562-4572, 2013.

\bibitem{Daniele13} D. Angelosante, G. B. Giannakis, N. D. Sidiropuolos, ``Sparse Parametric Models for Robust Nonstationary Signal Analysis,'' \emph{IEEE Signal Processing Mag.}, vol. 30, no. 6, pp. 64-73, 2013.

\bibitem{Balazs13} P. Balazs, M. Dorfler, M. Kowalski, B. Torresani, ``Adapted and Adaptive Linear Time-Frequency Representation,'' \emph{IEEE Signal Processing Mag.}, vol. 30, no. 6, pp. 20-31, 2013.

%\bibitem{Li19} L. Li and H. Cai, Q. Jiang and H. Ji, ``An empirical signal separation algorithm for multicomponent signals based on linear time-frequency analysis,'' \emph{Mechanical Systems and Signal Processing}, vol. 121, no. 4, pp. 791-809, 2019.

\bibitem{Huang09} N. E. Huang, Z. Wu, S. R. Long, K. C. Arnold, X. Chen and K. Blank, ``On Instantaneous Frequency'', \emph{Adv. Adapt. Data Anal.}, vol. 1, pp. 177-229, 2009.

\bibitem{Meignen07} S. Meignen and V. Perrier, ``A new formulation for empirical mode decomposition based on constraint optimization'', \textit{IEEE Signal Processing Letters}, vol. 14, pp. 932-935, 2007.

\bibitem{Pustelnik14} N. Pustelnik, P. Borgnat and P. Flandrin, ``Empirical mode decomposition revisited by multicomponent non-smooth convex optimization,'' \textit{Signal Processing}, vol. 102, pp. 313-331, 2014.

\bibitem{Lin09} L. Lin, Y. Wang, H. Zhou, ``Iterative filtering as an alternative algorithm for empirical mode decomposition,'' \emph{Adv. Adapt. Data Anal.}, Vol 1, no. 4, pp. 543–560, 2009.

\bibitem{Cicone16} C. Cicone, J. Liu, H. Zhou, ``Adaptive local iterative filtering for signal decomposition and instantaneous frequency analysis,'' \emph{Appl. Comput. Harmon. Anal.}, vol. 30, no. 2, pp. 243–261, 2011.

\bibitem{Hou11} T. Y. Hou, Z. Shi, ``Adaptive Data Analysis via Sparse Time-Frequency Representation,'' \emph{Adv. Adapt. Data Anal.}, vol. 3, no. 1, pp. 1-28, 2011.

\bibitem{Hou16} T. Y. Hou, Z. Shi, ``Sparse time-frequency decomposition based on dictionary adaptation,'' \emph{Phil. Trans. R. Soc. A}, vol. 374, pp. 20150192, 2016.

\bibitem{Wu09} Z. Wu and N. E. Huang, ``Ensemble empirical mode decomposition: a noise-assisted data analysis method,'' \emph{Adv. Adapt. Data Anal.}, vol. 1, no. 1, pp. 1-41, 2009.

\bibitem{Rehman13-AADA} N. Rehman, C. Park, N. E. Huang, and D. P. Mandic, ``EMD via MEMD multivariate noise-aided computation of standard EMD,'' \emph{Adv. Adapt. Data Anal.}, vol. 5, no. 2, pp. 1–25, 2013.

\bibitem{Lang20} X. Lang, N. Rehman, Y. Zhang, L. Xie, H. Su, ``Median ensemble empirical mode decomposition,'' \emph{Signal Process.}, vol. 176, 2020.


%

%\bibitem{Rilling08} G. Rilling and P. Flandrin, ``One or two frequencies? The Empirical Mode Decomposition answers,'' \emph{IEEE Trans. Signal Processing}, vol. 56, no. 1, pp. 85–95, 2008.

%------------------------- SST
\bibitem{SST_SPM13} F. Auger, P. Flandrin, Y. Lin, S. McLaughlin, S. Meignen, T. Oberlin, H. Wu, ``Time-Frequency Reassignment and Synchrosqueezing,'' \emph{IEEE Signal Process. Mag.}, vol. , pp. 32-41, 2013.


\bibitem{Thakur11} J. Thakur and H.-T. Wu, ``Synchrosqueezing based recovery of instantaneous frequency from nonuniform samples,'' \emph{SIAM J. Math. Anal.}, vol. 43, no. 5, pp. 2078–2095, 2011.

\bibitem{Thakur13} G. Thakur, E. Brevdo, N. S. Fuckar, and H.-T. Wu, ``The synchrosqueezing algorithm for time-varying spectral analysis: Robustness properties and new paleoclimate applications,'' \emph{Signal Process.}, vol. 93, no. 5, pp. 1079–1094, 2013.

\bibitem{Huang16} Z. Huang, J. Zhang, T. Zhao, and Y. Sun, ``Synchrosqueezing S-Transform and its Application in Seismic Spectral Decomposition,'' \emph{IEEE Trans. GeoSci. Remote Sens.}, vol. 54, no. 2, pp. 817-825, 2016.

\bibitem{daub15} I. Daubechies, Y. Wang, H. Wu, ``ConceFT: Concentration of frequency and time via a multitapered synchrosqueezed transform,'' \emph{Phil. Trans. R. Soc. A}, vol. 374, pp. 20150193, 2016.

\bibitem{Oberlin15} T. Oberlin, S. Meignen, and V. Perrier, ``Second-Order Synchrosqueezing Transform or Invertible Reassignment? Towards Ideal Time-Frequency Representations,'' \emph{IEEE Trans. Signal Process.}, vol. 63, no. 5, pp. 1335–1344, 2015.

\bibitem{Bahera18} R. Bahera, S. Meignen, T. Oberlin, ``Theoretical analysis of the second-order synchrosqueezing transform,'' \emph{Appl. Comput. Harmon. Anal.}, vol. 35, no. 2, pp. 379-404, 2018.

\bibitem{Pham17} D. Pham, S. Meignen, ``High-Order Synchrosqueezing Transform for Multicomponent Signals Analysis -- With an Application to Gravitational-Wave Signal,''  \emph{IEEE Trans. Signal Process.}, vol. 62, no. 12, pp. 3168-3178, 2017.

\bibitem{Yang18} H. Z. Yang, ``Statistical analysis of synchrosqueezed transforms,'' \emph{Appl. Comput. Harmon. Anal.}, vol. 45, no. 3, pp. 526-550, 2018.

\bibitem{Chui16} C. K. Chui and H. N. Mhaskar, ``Signal decomposition and analysis via extraction of frequencies,'' \emph{Appl. Comput. Harmon. Anal.}, vol. 40, no. 1, pp. 97-136, 2016.

\bibitem{Li20} L. Li, C. K. Chui, Q. Jian``Direct Signal Separation Via Extraction of Local Frequencies with Adaptive Time-Varying Parameters'', \emph{arXiv:2010.01866}, 2020.

\bibitem{Meignen17} S. Meignen, D. Pham, S. McLaughlin, ``On Demodulation, Ridge Detection, and Synchrosqueezing for Multicomponent Signals,'' \emph{IEEE Trans. Signal Process.}, vol. 65, no. 8, pp. 2093-2103, 2017.

\bibitem{Laurent20} N. Laurent, S. Meignen, ``A Novel Approach for Ridge Detection and Mode Retrieval of Multicomponent Signals Based on STFT,'' \emph{arXiv:2009.13123v1}, 2020.

%\bibitem{Jiang17} Q. Jiang and B. W. Suter, ``Instantaneous frequency estimation based on synchrosqueezing wavelet transform,'' \emph{Signal Process.}, vol. 138, pp.167-181, 2017.



%----------------------------------------- VMD based

\bibitem{VMD14} K. Dragomiretskiy, D. Zosso, ``Variational Mode Decomposition'',  \emph{IEEE Trans. Signal Processing}, vol. 62, no. 3, pp. 531-544, 2014.

\bibitem{NCMD18} S. Chen, X. Dong, Z. Peng, W. Zhang, G. Meng, ``Nonlinear Chirp Mode Decomposition'',  \emph{IEEE Trans. Signal Processing}, vol. 65, no. 22, pp. 6024-6037, 2017.

%---------------------- ICA based approaches
\bibitem{Comon94} P. Comon, ``Independent Component Analysis, a new concept?,'' \emph{Signal Process.}, vol. 36, pp. 287-314, 1994.
36, pp.287-314

\bibitem{Lee99} D. D. Lee and H. S. Seung, ``Learning the parts of objects with nonnegative matrix factorization,'' \emph{Nature}, vol. 401, pp. 788–791, 1999.

\bibitem{Smaragdis14} P. Smaragdis, C. Févotte, G. J. Mysore, N. Mohammadiha, M. Hoffman, ``Static and Dynamic Source Separation Using Nonnegative Factorizations,'' \emph{IEEE Signal Processing Mag.}, vol. 32, no. 3, pp. 66-75, 2014.

\bibitem{Broomhead86} D. Broomhead and G. King, ``Extracting qualitative dynamics from experimental data,'' \emph{Physica D}, vol. 20, pp. 217–236, 1986.

\bibitem{Schmid10} P. J. Schmid, ``Dynamic mode decomposition of numerical and experimental data,'' \emph{J. Fluid Mech.}, vol. 656, pp. 5–28, 2010.

\bibitem{Fland18} J. Harmouche, D. Fourer, F. Auger, P. Borgnat, P. Flandrin, ``The Sliding Singular Spectrum Analysis: a Data-Driven Non-Stationary Signal Decomposition Tool,'' \emph{IEEE Trans. Signal Process.}, vol. 66, no. 1, pp. 251-263, 2018.

\bibitem{LTFRS18} C. Févotte, M. Kowalski, ``Estimation With Low-Rank Time–Frequency Synthesis Models,''  \emph{IEEE Trans. Signal Process.}, vol. 66, no. 15, pp. 4121-4132, 2018.

%\bibitem{Amin98} A. Belouchrani, M. G. Amin, ``Blind Source Separation Based on Time–Frequency Signal Representations,'' \emph{IEEE Trans. Signal Process.}, vol. 46, no. 11, pp. 2888-2897, 2017.

%------------------------ Multivariate
\bibitem{Rehman09} N.~Rehman and D.~P.~Mandic, ``Multivariate Empirical Mode Decomposition,'' \emph{Proceedings of the Royal Society A}, vol.~466, no.~2117, pp.~1291-1302,~2010.

\bibitem{Rehman10} N. Rehman and D. P. Mandic, ``Empirical Mode Decomposition for Trivariate Signals,'' \emph{IEEE Trans. Signal Processing}, vol. 58, no. 3, pp. 1059-1068, 2010.

\bibitem{Rehman11} N. Rehman and D. P. Mandic, ``Filter Bank Property of Multivariate Empirical Mode Decomposition'', \emph{IEEE Trans. Signal Processing}, vol. 59, no. 5, pp. 2421-2426, 2011.




%
\bibitem{Cicone19} A. Cicone, ``Multivariate Fast Iterative Filtering for the decomposition of nonstationary signals,'' \emph{arXiv: 1902.04860}, 2019.

\bibitem{Rehman19} N. Rehman and H. Aftab, ``Multivariate Variational Mode Decomposition,'' \emph{IEEE Trans. Signal Process.}, vol. 67, no. 3, pp. 6039-6052, 2019.

\bibitem{Chen20} Q. Chen, L. Xie, H. Su, ``Multivariate nonlinear chirp mode decomposition,'' \emph{Signal Process.}, vol. 176, 2020.

\bibitem{Ali15} A. Ahrabian, D. Looney, L. Stankovic, D. P. Mandic, ``Synchrosqueezing-based time-frequency analysis of multivariate data,'' \emph{Signal Process.}, vol. 106, pp. 331-341, 2015.

\bibitem{MEWT18} O. Singh, R. K. Sunkaria, ``An empirical wavelet transform based approach for multivariate data processing application to cardiovascular physiological signals,'' \emph{Bio Alg. Med. Syst.}, vol. 14, no. 4, 2018.

\bibitem{Jain20} S. Jain, R. Panda, R. K. Tripathy, ``Multivariate Sliding-Mode Singular Spectrum Analysis for the Decomposition of Multisensor Time Series,'' \emph{IEEE Sens. Lett.}, vol. 4, no. 6, pp. 2475-147, 2020.

\bibitem{Stan20} L. Stankovic, M. Brajovi, M. Dakovi, D. P. Mandic, ``On the decomposition of multichannel nonstationary multicomponent signals,'' \emph{Signal Process.}, vol. 167, pp. 107261, 2020.

%----------------------- Nonconvex
\bibitem{Boyd04} S. Boyd, L. Vandenberghe, \emph{Convex Optimization}. New York, NY: Cambridge University Press, 2004.

\bibitem{Candes10}E. Candès and T. Tao, ``The power of convex relaxation: Near-optimal matrix completion,'' \emph{IEEE Trans. Inf. Theory}, vol. 56, no. 5, pp. 2053–2080, 2010.

\bibitem{Candes11} E. J. Candès, X. Li, Y. Ma, and J. Wright, ``Robust principal component analysis?,'' \emph{J. ACM}, vol. 58, no. 3, pp. 11:1–11:37, 2011.

\bibitem{Chandrasekaran11} V. Chandrasekaran, S. Sanghavi, P. Parrilo, and A. Willsky, ``Rank sparsity incoherence for matrix decomposition,'' \emph{SIAM J. Optim.}, vol. 21, no. 2, pp. 572–596, 2011.

\bibitem{Ahmad14} A. Ahmed, B. Recht, and J. Romberg, ``Blind deconvolution using convex programming,'' \emph{IEEE Trans. Inf. Theory}, vol. 60, no. 3, pp. 1711–1732, 2014.

\bibitem{Chi18} Y. Chen and Y. Chi, ``Harnessing structures in big data via guaranteed low-rank matrix estimation: Recent theory and fast algorithms via convex and nonconvex optimization,'' \emph{IEEE Signal Process. Mag.}, vol. 35, no. 4, pp. 14–31, Jul. 2018.

\bibitem{Jain17} P. Jain and P. Kar, ``Non-convex optimization for machine learning,'' \emph{Foundations Trends Machine Learn.}, vol. 10, no. 3–4, pp. 142–336, 2017.

\bibitem{Chi19} Y. Chi, Y. M, Lu, Y. Chen, ``Nonconvex Optimization Meets Low-Rank Matrix Factorization: An Overview,'' \emph{IEEE Trans. Signal Proces.}, vol. 67, no. 20, pp. 5239-5269, 2019.

\bibitem{cond19} W. Zhang, D. Yang, H. Wang, ``Data-Driven Methods for Predictive Maintenance of Industrial Equipment:
A Survey,'' \emph{IEEE Syst. J.}, vol. 13, pp. 2213–2227, 2019.


\bibitem{Morse20} K. E. Morse, S. C. Bagley and N. H. Shah,``Estimate the hidden deployment cost of predictive models to improve patient care,'' \emph{Nat. Med.}, vol. 26, pp. 18–19, 2020.

\bibitem{Mandic17} V. Goverdovsky, W. von Rosenberg, T. Nakamura et al. ``Hearables: Multimodal physiological in-ear sensing,'' \emph{Sci Rep}, vol. 7, no. 6948, 2017.

\bibitem{Sharma20} P. Sharma, X. Hui, J. Zhou et al. ``Wearable radio-frequency sensing of respiratory rate, respiratory volume, and heart rate,'' \emph{Digit. Med.}, vol. 3, no. 98, 2020.

\bibitem{Vaswani20} N. Vaswani, ``Nonconvex Structured Phase Retrieval: A Focus on Provably Correct Approaches,'' \emph{IEEE Signal Processing Mag.}, vol. 37, no. 5, pp. 67-77, 2020.

\bibitem{Looney12} D. Looney, P. Kidmose, C. Park, M. Ungstrup, M. L. Rank, K. Rosenkranz and D. P. Mandic, ``The In-the-Ear Recording Concept: User-Centered and Wearable Brain Monitoring,'' \emph{IEEE Pulse}, vol. 3, no. 6, pp. 32-42, 2012.
\bibitem{Aimoni18} C. Aimoni, L. Crema, S. Savini, et al. ``Hearing threshold estimation by auditory steady state responses (ASSR) in children'', \emph{Acta Otorhinolaryngol Ital.}, vol. 38, pp. 361-368, 2018.
\bibitem{Wu20} H-T Wu, ``Current state of nonlinear-type time–frequency analysis and applications to high-frequency biomedical signals,'' \emph{Current Opinion in Systems Biology}, vol. 23, pp. 8-11, 2020.
\bibitem{Zhang17} X. S. Zhang and F. Wang, ``Signal Processing for Finance, Economics, and Marketing: Concepts, framework, and big data applications,'' \emph{IEEE Signal Process. Mag.}, vol. 34, no. 3, pp. 14-35, 2017.
\bibitem{Takeuchi20} D. Takeuchi, K. Yatabe, Y. Koizumi, Y. Oikawa, N. Harada,``Invertible DNN-based nonlinear time-frequency transform for speech enhancement,'' \emph{arXiv:1911.10764v2}, 2020.
\bibitem{Wong18} L. Wong, Y. Chen, Q. Wang, V. Kuehnel, ``Efficacy of a Hearing Aid Noise Reduction Function,'' \emph{Trends Hear.}, vol. 22, 2018.


% ------------------------ Ear EEG, Hyperscanning

%\bibitem{Looney12} D. Looney, P. Kidmose, C. Park, M. Ungstrup, M. L. Rank, K. Rosenkranz, D. Mandic, ``The In-the-Ear Recording Concept: User-Centered and Wearable Brain Monitoring,'' \emph{IEEE Pulse}, vol. 3, no. 6, pp. 32-42, 2012.

%\bibitem{Kidmose13} P. Kidmose, D. Looney, M. Ungstrup, M. L. Rank and D. P. Mandic, ``A Study of Evoked Potentials From Ear-EEG,'' \emph{IEEE Trans. Biomedical Eng.}, vol. 60, no. 10, pp. 2824-2830, 2013.

%\bibitem{Kappel19} S. L. Kappel, M. L. Rank, H. O. Toft, M. Andersen and P. Kidmose, ``Dry-Contact Electrode Ear-EEG,'' \emph{IEEE Trans. Biomedical Eng.}, vol. 66, no. 1, pp. 150-158, 2019.

%

%\bibitem{Aimoni18} C. Aimoni, L. Crema, S. Savini, et al. ``Hearing threshold estimation by auditory steady state responses (ASSR) in children'', \emph{Acta Otorhinolaryngol Ital.}, vol. 38, pp. 361-368, 2018.



%\bibitem{Rehman13} D. P. Mandic, N. Rehman, Z. Wu, N. E. Huang, ``Empirical Mode Decomposition-Based Time-Frequency Analysis of Multivariate Signals: The Power of Adaptive Data Analysis'', \emph{IEEE Signal Process. Mag.}, vol. 30, pp. 74-86, 2013.

\bibitem{ChenML19} J. Chen and X. Ran, ``Deep learning with edge computing: A review,'' \emph{Proc. IEEE}, vol 107, pp. 1655-1674, 2019.

\bibitem{Yonina20} N. Shlezinger, J. Whang, Y. C. Eldar and A. G. Dimakis, ``Model based deep learning'', \emph{arXiv:2012.08405v1}, 2020.

%--------------- Basin of att

\bibitem{Jain13} P. Jain, P. Netrapalli, and S. Sanghavi, ``Low-rank matrix completion using alternating minimization,'' \emph{in Proc. 45th Annu. ACM Symp. Theory Comput.}, ACM, 2013, pp. 665–674.

\bibitem{Jain16} Y. Cherapanamjeri, K. Gupta, P. Jain, ``Nearly optimal robust matrix completion,'' \emph{in Proc. Int. Conf. Machine Learning.}, 2016.

\bibitem{Jain14} P. Netrapalli, U. N. Niranjan, S. Sanghavi, A. Anandkumar and P. Jain, ``Nonconvex robust PCA,'' \emph{in Proc. Conf. Neural Inf. Process. Systems}, 2014, pp. 1107-1115.

\bibitem{Keshavan10} R. H. Keshavan, A. Montanari, and S. Oh, ``Matrix completion from a few entries,'' \emph{IEEE Trans. Inf. Theory}, vol. 56, no. 6, pp. 2980–2998, 2010.

\bibitem{Chen15} Y. Chen, M. J. Wainwright, ``Fast low-rank estimation by projected gradient descent: General statistical and algorithmic guarantees,'' \emph{arXiv:1509.03025}, 2015.

\bibitem{Candes15} E. Candès, X. Li, and M. Soltanolkotabi, ``Phase retrieval via Wirtinger flow: Theory and algorithms,'' \emph{IEEE Trans. Inf. Theory}, vol. 61, no. 4, pp. 1985–2007, 2015.

\bibitem{Zhang16} H. Zhang, Y. Chi, Y. Liang, ``Provable non-convex phase retrieval with outliers: Median truncated Wirtinger flow,'' \emph{in Proc. Int. Conf. Mach. Learn.}, 2016, pp. 1022–1031.

%------------------ no spurious minima

\bibitem{Ge16} R. Ge, J. D. Lee, T. Ma, ``Matrix completion has no spurious local minimum,'' \emph{in Proc. Adv. Neural Inf. Process. Syst.}, 2016, pp. 2973–2981.

\bibitem{Sun16} R. Sun, Z.-Q. Luo, ``Guaranteed matrix completion via non-convex factorization,'' \emph{IEEE Trans. Inf. Theory}, vol. 62, no. 11, pp. 6535–6579, 2016.

\bibitem{Tu16} S. Tu, R. Boczar, M. Simchowitz, M. Soltanolkotabi, B. Recht, ``Low rank solutions of linear matrix equations via Procrustes flow,'' \emph{in Proc. Int. Conf. Mach. Learn.}, 2016, pp. 964–973.

\bibitem{Bhojanapalli16} S. Bhojanapalli, B. Neyshabur, N. Srebro, ``Global optimality of local search for low rank matrix recovery,'' \emph{in Proc. Adv. Neural Inf. Process. Syst.}, 2016, pp. 3873–3881.

%\bibitem{Chen17} Y. Chen, E. Candès, ``Solving random quadratic systems of equations is nearly as easy as solving linear systems,'' \emph{Commun. Pure Appl. Math.}, vol. 70, no. 5, pp. 822–883, 2017.

\bibitem{Ge15} R. Ge, F. Huang, C. Jin, Y.Yuan, ``Escaping from saddle points-online stochastic gradient for tensor decomposition,'' \emph{in Proc. Conf. Learn. Theory}, pp. 797–842, 2015.

%-------------
%\bibitem{Ozerov10} A. Ozerov and C. Fevotte, ``Multichannel nonnegative matrix factorization in convolutive mixtures for audio source separation,'' \emph{IEEE Trans. Audio Speech Lang. Process.}, vol. 18, no. 3, pp. 550–563, 2010.

\bibitem{Fevotte11} C. Fevotte and J. Idier, ``Algorithms for nonnegative matrix factorization with the $\beta$-divergence,'' \emph{Neural Comput.}, vol. 23, no. 9, pp. 2421–2456, 2011.

\bibitem{Emiya18} V. Emiya, R. Hamon and C. Chaux, ``Being Low-Rank in the Time-Frequency Plane,'' \emph{in Proceedings IEEE (ICASSP)}, Calgary, pp. 4659-4663, 2018.

%\bibitem{Rehman13-AADA} N. Rehman, C. Park, N. E. Huang, and D. Mandic, ``EMD via MEMD multivariate noise-aided computation of standard EMD,'' \emph{Adv. Adapt. Data Anal.}, vol. 5, no. 2, pp. 1–25, 2013.

%\bibitem{Rehman11} N. Rehman and D. Mandic, ``Filter Bank Property of Multivariate Empirical Mode Decomposition'', \emph{IEEE Trans. Signal Processing}, vol. 59, no. 5, pp. 2421-2426, 2011.

%--------------------------???
\bibitem{Boyd11} S. Boyd, N. Parikh, E. Chu, B. Peleato, and J. Eckstein, ``Distributed Optimization and Statistical Learning via the Alternating Direction Method of Multipliers,'' \emph{Found. Trends Mach. Learn.}, vol. 3, pp. 1-22, 2011.

\bibitem{Chen19} Y. Chen, Y. Chi, J. Fan, and C. Ma, ``Gradient descent with random initialization: fast global convergence for nonconvex phase retrieval,'' \emph{Math. Program.}, vol. 176, no. 1-2, pp. 5-37, 2019.

\bibitem{NGD2} Z. Allen-Zhu, ``Natasha 2: Faster non-convex optimization than SGD,'' \emph{in Proc. Neural Inf. Process. Syst.}, 2018, pp. 2675–2686.

\bibitem{NGD3} Y. Xu, J. Rong, and T. Yang, ``First-order stochastic algorithms for escaping from saddle points in almost linear time,'' \emph{in Proc. Adv. Neural Inf. Process. Syst.}, 2018, pp. 5530–5540.

\bibitem{NGD4} Z. Allen-Zhu and Y. Li, ``Neon2: Finding local minima via first-order oracles,'' \emph{in Proc. Neural Inf. Process. Syst.}, 2018, pp. 3716–3726.
    
    \bibitem{Jin17} C. Jin, R. Ge, P. Netrapalli, S. M. Kakade, and M. I. Jordan, ``How to escaping saddle points efficiently,'' \emph{in Proc. Int. Conf. Machine Learn.}, 2017, pp. 1724-1732.

%--------------------- Denoising

%\bibitem{Donoho95} D. Donoho, ``De-noising by soft-thresholding,'' \emph{IEEE Trans. Inf. Theory}, vol. 41, no. 3, pp. 613–627, 1995.

%\bibitem{Rehman17} N. Rehman, Z. Abbas, A. Asif, A. Javed, K. Naveed and D. P. Mandic,   ``Translation invariant multi-scale signal denoising based on goodness-of-fit tests,'' \emph{Signal Process.}, vol. 121, pp. 230-244, 2017.

\bibitem {Hao17} H. Hao, H.L. Wang and N. Rehman, ``A joint framework for multivariate signal denoising using multivariate empirical mode decomposition,'' \emph{Signal Process.}, vol. 135, pp. 263-273, 2017.

\bibitem{Rehman19SPL} N. Rehman, B. Khan and K. Naveed ``Multivariate Signal Denoising using Mahalanobis Distance,'' \emph{IEEE Signal Processing Lett.}, vol. 26, pp. 1408-1412, 2019.

\bibitem{Rehman20} K. Naveed and N. Rehman, ``Wavelet based multivariate signal denoising using Mahalanobis distance and EDF statistics,'' \emph{IEEE Trans. Signal Process.}, vol. 68, pp. 5997-6010, 2020.

\bibitem{Park12} C. Park, D. Looney, P. Kidmose, M. Ungstrp, D. P. Mandic, ``Time-frequency analysis of EEG asymmetry using bivariate empirical mode decomposition,'' \emph{IEEE Trans. Neural Syst. Rehabilitation Eng.}, vol. 19, no. 4, pp. 366-373, 2011.

\bibitem{Hyperscanning14} F. Babilonia, L. Astolfia, ``Social neuroscience and hyperscanning techniques: Past, present and future,'' \emph{Neuroscience  Biobehavioral Rev.}, vol . 44, pp. 76-93, 2014.

\bibitem{Parra19} L. C. Parra, S. Haufe, J. P. Dmochowski, ``Correlated Components Analysis -- Extracting Reliable Dimensions in Multivariate Data,'' \emph{Neurons Behav. Data Anal. Theory (NBDT)}, arXiv:1801.08881, 2019.

\end{thebibliography}


